Everyday Finger: A Robotic Finger that Meets the Needs of Everyday Interactive Manipulation

We provide the mechanical and dynamical requirements for a robotic finger capable of performing thirty diverse everyday tasks. To match these requirements, we present a finger design based on series-elastic actuation that we call the everyday finger. Our focus is to make the fingers as compact as possible while achieving the desired performance. We evaluated everyday fingers by constructing a two-finger robotic hand that was tested on various performance parameters and tasks like picking and placing dishes in a rack, picking thin and flat objects like paper and delicate objects such as strawberries. Videos are available at the project website: https://sites.google.com/view/everydayfinger.

==> Extras.tex <==

\subsection{Additional features for a great robotic hand}

A great robotic hand is one that can take advantage of the current state of the art control/software technologies. This great hand will also have a tune-able stiffness, force sensing, tactile sensing, and the capability for simulation. Many previous attempts at robotic hands have prioritized hardware goals, and have fallen short when it comes to integrating with the rest of the technology stack. Reinforcement learning methods have proven to be effective in controlling dexterous hands in re-orientation \cite{}, piano playing \cite{}, and more. Training these models in virtual environments can dramatically cut costs since there's no need for physical hardware. For the foreseeable future, these strategies are poised to dominate—until the advent of more efficient learning methods requiring fewer demos and advanced visual and language models which would enable training to happen in the real world. 

With the current capabilities of computing in robots, the operational frequency of trained networks peaks at around 50Hz. This control frequency is insufficient for ensuring stable contacts if commanding positions. In one time step, contact could be lost and an object can drop a few cm. Hence, \textbf{adjustable stiffness}, achieved through physical means or through high frequency impedance control + transmission transparency, becomes vital: it permits dynamic modulation of the control intensity, enabling the hand to manage both large and small loads while maintaining consistent contact. \textbf{Force sensing} allows for compliance to be achieved via impedance control, and also provides feedback for a high-level controller. \textbf{Tactile Sensing} has proven to be critical for obtaining precision poses of small objects that may be partially occluded from cameras 
\cite{}, so it's necessary for manipulating small objects such as in small bolt insertion. The \textbf{capability for accurate and fast simulation} is also required in order to use Sim2Real methods. While a soft hand may give us many of the above desired characteristics, it is impractical to train a neural network on a simulation of it, as the speed of an accurate enough simulation would be slower than real time.

